Evidence-Focused Fact Summarization for Knowledge-Augmented Zero-Shot Question Answering

Recent studies have investigated utilizing Knowledge Graphs (KGs) to enhance Quesetion Answering (QA) performance of Large Language Models (LLMs), yet structured KG verbalization remains challengin. Existing methods, such as triple-form or free-form textual conversion of triple-form facts, encounter several issues. These include reduced evidence density due to duplicated entities or relationships, and reduced evidence clarity due to an inability to emphasize crucial evidence. To address these issues, we propose EFSum, an Evidence-focused Fact Summarization framework for enhanced QA with knowledge-augmented LLMs. We optimize an open-source LLM as a fact summarizer through distillation and preference alignment. Our extensive experiments show that EFSum improves LLM's zero-shot QA performance, and it is possible to ensure both the helpfulness and faithfulness of the summary.

==> 010introduction_original.tex <==

% 1. LLM prompting with knowledge augmention for QA.
Large Language Models (LLMs) have shown remarkable zero-shot capabilities but often produce factual errors, known as \textit{hallucinations}, particularly in knowledge-intensive tasks like Question Answering (QA). 
This happens because the static knowledge within LLM parameters may be incomplete, incorrect, or outdated, failing to keep pace with evolving real-world knowledge.
Recent studies aim to remedy this by integrating external knowledge into LLMs~\cite{Karpukhin2020DensePR, Min2019KnowledgeGT}.
For instance, in open-domain QA frameworks, relevant passages are retrieved from document collections (e.g., Wiki corpus), which are then used to augment LLMs as contextual knowledge~\cite{ma-etal-2022-open}. 
By leveraging the external knowledge, LLMs are able to generate factual answers without the need to update their parameters.


% 2. Challenges of utilizing triples for knowledge-augmented prompting.
Recently, there have been several attempts to consider Knowledge Graphs (KGs) as the knowledge source to augment LLMs for enhanced performance in knowledge graph QA (KGQA)~\cite{baek2023knowledgeaugmented,wu2023retrieve,sen-etal-2023-knowledge}.
The primary challenge lies in the structured nature of KGs, which consist of facts presented in a triple format (head entity, relation, tail entity).
Consequently, existing methods typically involve retrieving a set of relevant facts based on semantic similarity to a given question, followed by a process of verbalization into textual form for LLM prompting.
Upon retrieving the relevant facts, one verbalization strategy is simply concatenating the facts in their \textit{triple-form} text~\cite{baek2023knowledgeaugmented}, while the other entails converting them into semantically-coherent textual description (i.e., \textit{free-form} text) through the distillation of LLM's ability to generate text from KGs~\cite{wu2023retrieve}.

% After filtering out irrelevant facts, they transform the set of facts into the knowledge contexts, which would be fed into the LM for zero-shot QA tasks.
% To this end, they first retrieve triples based on their semantic similarity to an input question, and then prepend the most relevant triples to the input question in the form of the prompt.
% They first retrieve the most relevant facts to a given query from external knowledge graphs (KGs), by either dense retrieval based on the relevance computed by pretrained language model~\cite{} or multi-hop matching~\cite{}.
% Some approaches linearize triples for verbalization through concatenation. 

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{FIG/pipeline.pdf}
    \caption{The QA pipeline based on LLM prompting, augmented with relevant facts from KGs. Our fact summarization improves both density and clarity of evidence within contextual knowledge for enhanced QA.}
    \label{fig:pipeline}
\end{figure}

% 3. 
Despite their remarkable efficacy, existing verbalization strategies for providing contextual knowledge exhibit critical limitations.
\textbf{(1) Low density of evidence}: 
Both concatenation and linearization of the facts~\cite{baek2023knowledgeaugmented, wu2023retrieve} are highly likely to include duplicated entities or relations due to limited flexibility;
this eventually degrades the density of useful evidence within the contextual knowledge, hindering the ability to answer questions effectively.
\textbf{(2) Low clarity of evidence}:
While contextual knowledge describes factual information, they often fail to highlight the evidence necessary for answering questions. 
This lack of focus can lead to noise from irrelevant facts, which can detrimentally impact the LLM's ability to provide accurate answers. 
For this reason, even when sufficient evidence (or an exact answer span) is presented in the knowledge context, LLMs may struggle to properly identify it.

% 4.
To address the aforementioned challenges, we introduce a novel \textbf{\proposed} framework, \textbf{E}vidence-focused \textbf{F}act \textbf{Sum}marization for enhanced QA with knowledge-augmented LLM prompting. 
The key idea is transforming the set of facts into plausible and coherent \textit{summary} while highlighting evidence and filtering out noise given a question;
this ensures that the summaries maintain a high density and clarity of evidence, facilitating effective QA (Figure~\ref{fig:pipeline}).
The most straightforward solution to this summarization is prompting LLMs with the detailed instruction.
However, LLM-generated summaries often omit crucial evidence (such as answer spans), resulting in \textit{information loss}, or include information that cannot be inferred from retrieved facts, leading to \textit{extrinsic hallucination}.

For enhanced summary quality, we optimize an open-source LLM as a fact summarizer in two steps: LLM distillation and preference alignment (Figure~\ref{fig:framework}).
During the first step, we train our fact summarizer by using the reference summaries obtained through LLM prompting.
Subsequently, in the second step,
we refine our summarizer to better align with the task-specific preference related to QA.
To this end, we introduce two preference criteria for the summary candidates:
\textit{helpfulness} evaluates LLMs can correctly answer the question based on the summary, and \textit{faithfulness} assesses the factual consistency of the summary in relation to the provided set of facts.
By selecting pairs of preferred and dispreferred summaries based on these criteria, we further fine-tune the summarizer through direct preference optimization (DPO)~\cite{rafailov2023direct}.
In the end, \proposed is capable of generating summaries that are both helpful for QA and faithful to the given facts.

% 5.
Extensive experiments on two QA benchmark datasets validate the effectiveness of our evidence-focused fact summarization in improving LLM's zero-shot QA performance. 
Our approach significantly improves the zero-shot QA performance of LLMs, while also enhancing the helpfulness and faithfulness of the generated fact summaries.

% Our main contributions are as follows:
% \begin{itemize}
%     \item We incorpoate an additional summarization process into knowledge-augmented zero-shot QA pipeline for higher density and obivousness of evidence.
    
%     \item We present a novel \proposed to generate concise summaries that are faithful to the input facts and also helpful to make LLMs answer the question.
    
%     \item Our experiments demonstrate that \proposed outperforms the baseline methods, showing remarkable robustness on the retrieved facts. The generated summary effectively highlights the evidence for QA task. 
% \end{itemize}

==> 041maintable_old.tex <==

\begin{table*}[thbp]
\label{main_table}
\centering
\resizebox{.99\textwidth}{!}{
\begin{tabular}{clcccccccccccc}
\toprule
         & \multicolumn{1}{r}{QA model}               & \multicolumn{4}{c}{GPT-3.5-turbo}                  & \multicolumn{4}{c}{Flan-T5-XL(3B)}                    & \multicolumn{4}{c}{Llama-7B-chat}                     \\ \cline{3-14} 
         & \multicolumn{1}{r}{Prompt}                 & \multicolumn{2}{c}{F1} & \multicolumn{2}{c}{Acc}   & \multicolumn{2}{c}{F1}    & \multicolumn{2}{c}{Acc}   & \multicolumn{2}{c}{F1}    & \multicolumn{2}{c}{Acc}   \\ \cline{3-14} 
         & \multicolumn{1}{r}{\# of Retrived Triples} & K=10       & K=30      & K=10        & K=30        & K=10         & K=30       & K=10        & K=30        & K=10         & K=30       & K=10        & K=30        \\ \midrule
\multirow{6}{*}{WebQSP}  & No knowledge                               & \multicolumn{2}{c}{}   & \multicolumn{2}{c}{0.506} & \multicolumn{2}{c}{0.468} & \multicolumn{2}{c}{0.409} & \multicolumn{2}{c}{0.162} & \multicolumn{2}{c}{0.539} \\
         & KAPING                                     &            &           & 0.547       & 0.55        & 0.446        & 0.512      & 0.397       & 0.455       & 0.309        & 0.082      & 0.499       & 0.516       \\
         & KG2Text                                    &            &           &             &             &              &            &             &             &              &            &             &             \\
         & Rewrite                                    &            &           &             & 0.6         & 0.489        & 0.533      & 0.425       & 0.473       & 0.274        & 0.286      & 0.474       & 0.47        \\
         & FQSum w/ LLM(ours)                         &            &           & 0.565       & 0.596       & 0.461        & 0.507      & 0.399       & 0.452       & 0.266        & 0.282      & 0.462       & 0.484       \\
         & FQSum w/ Distilled(ours)                   &            &           & 0.572       & 0.607       & 0.479        & 0.52       & 0.407       & 0.478       & 0.258        & 0.286      & 0.492       & 0.542       \\ \midrule
\multirow{6}{*}{Mintaka} & No knowledge                               & \multicolumn{2}{c}{}   & \multicolumn{2}{c}{0.54}  & \multicolumn{2}{c}{}      & \multicolumn{2}{c}{0.211} & \multicolumn{2}{c}{}      & \multicolumn{2}{c}{0.492} \\
         & KAPING                                     &            &           &             & 0.553       &              &            & 0.286       & 0.416       &              &            & 0.379       & 0.408       \\
         & KG2Text                                    &            &           &             &             &              &            &             &             &              &            &             &             \\
         & Rewrite                                    &            &           &             & 0.572       &              &            & 0.319       & 0.343       &              &            & 0.357       & 0.366       \\
         & \proposed w/ LLM(ours)                         &            &           &             & 0.553       &              &            & 0.292       & 0.321       &              &            & 0.325       & 0.353       \\
         & \proposed w/ Distilled(ours)                   &            &           &             & 0.541       &              &            & 0.289       & 0.313       &              &            & 0.424       & 0.428       \\ \bottomrule
\end{tabular}}
\end{table*}
